Early Identification of Services in HTTPS Traffic

Traffic monitoring is essential for network management tasks that ensure security and QoS. However, the continuous increase of HTTPS traffic undermines the effectiveness of current service-level monitoring that can only rely on unreliable parameters from the TLS handshake (X.509 certificate, SNI) or must decrypt the traffic. We propose a new machine learning-based method to identify HTTPS services without decryption. By extracting statistical features on TLS handshake packets and on a small number of application data packets, we can identify HTTPS services very early in the session. Extensive experiments performed over a significant and open dataset show that our method offers a good accuracy and a prototype implementation confirms that the early identification of HTTPS services is satisfied.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> TLS-Background.tex <==
%Nowadays, TLS is the key encryption protocol over Internet. 
%The TLS primary goal is to establish a secure channel, so a potential third party can not intercept the communication. Therefore, it is used widely in applications like HTTP, FTP and SMTP to protect their data exchanges. 

The HTTPS is the predominant protocol over the web since it vehiculates rich and various services (audio-video streaming, online storage, etc.). Technically, HTTP protocol is used on top of a TLS connection. So, to establish an HTTPS connection, client and server must first complete a TLS handshake protocol. The handshake protocol is of prime importance because it defines many configuration aspects such as managing cipher suite negotiation, server/client authentication, and session key exchange. During cipher suite negotiation, client and server agree about a cipher suite that will be used to exchange data \cite{dierks2008transport}. Figure \ref{tlshandshake} details the sequence of the TLS handshake protocol messages.
%In this paper, the messages exchanged during the TLS handshake are used to identify HTTPS services in real-time.

\begin{enumerate}
%\itemsep0em
\item The \texttt{ClientHello} message contains the usable cipher suites, supported extensions (e.g. SNI) and a random number.
\item The \texttt{ServerHello} message holds the selected cipher, supported extensions and a random number.
\item The \texttt{ServerCertificate} message contains a certificate with a server public key.
\item The \texttt{ServerHelloDone} indicates the end of the \texttt{ServerHello} and associated messages. If the client receives a request for its certificate, it sends\\ a \texttt{ClientCertificate} message. 
\item Based on the server random number, the client generates a random Pre-Master Secret, encrypts it with the public key given in the server's certificate and sends it to the server.
\item Both client and server generate a master secret from the Pre-Master Secret and exchanged random values. 
\item The client and the server exchange \texttt{ChangeCipherSpec} to start using the new keys for encryption.
\item The client sends the \texttt{Finished} message to verify that the key exchange and authentication processes were successful.
\item The server sends the \texttt{Finished} message to the client to end the handshake phase.
\end{enumerate}

Once both sides have received and validated the \texttt{Finished} message from its peer, they can exchange encrypted application data over the new TLS connection. 

\begin{figure}
\centering
\includegraphics[scale=0.39]{images/TLS-Handshake-new.eps}
\caption{TLS handshake protocol messages sequence}
\label{tlshandshake}
\end{figure}

%\begin{table}[]
%\setlength{\belowcaptionskip}{-10pt}
%\centering
%\caption{TLS Handshake protocol messages}
%\label{tlsmessage}
%\begin{tabular}{|l|l|}
%\hline
%\textbf{Message} & \textbf{Parameters} \\ \hline \hline
%ClientHello & \begin{tabular}[c]{@{}l@{}}Version, Random, SessionID, Cipher suite, \\ Compression methods, Extensions \end{tabular} \\ \hline
%ServerHello & \begin{tabular}[c]{@{}l@{}}Version, Random, SessionID, Selected\\ Ciphers, Compression methods, Extension\end{tabular} \\ \hline
%Certificate & Chain of X509 certificates \\ \hline
%Server Key Exchange & Parameters, Signature \\ \hline
%Certificate Request & Type, Authorities \\ \hline
%Server done & Null \\ \hline
%Certificate Verify & Signature \\ \hline
%Client key Exchange & Parameters, Signature \\ \hline
%Finished & Hash value \\ \hline
%\end{tabular}
%\end{table}

==> TLS-Protocol.tex <==
\subsection{Protocol History}
Nowadays, SSL and TLS protocols are known as the key encrypted protocols over Internet. Those two names come from the protocol history. At the end of 1994 Netscape included the support of the second version of SSL (SSL 2.0) in Netscape Navigator after solving many issues with the first version which was just used inside Netscape Corporation. %The presence of a web browser supporting encryption techniques opened the door for a competition between companies to embed encryption in their own.
In response, Microsoft also introduced in 1995 an encryption protocol named Private Communication Technology (PCT) that was very close to SSL 2.0 \cite{oppliger2009ssl}. The publication of two concurrent encryption protocols created a lot of confusion in the security community, since applications needed to support both for interoperability reasons. To resolve this issue, the IETF formed a working group in 1996 to standardize a unified TLS protocol. After a long discussion with the related parties, the first version of standard protocol (TLS 1.0) appeared in January 1999. In April 2006, the TLS protocol version 1.1 (TLS 1.1) was released, followed by TLS 1.2 in August 2008 which is specified in the RFC5246 \cite{dierks71rfc} standard. The most recent version of TLS is TLS 1.3, but is still a draft. The new version has the same specifications but with improvements of the encryption algorithms parameters and the handshake \cite{tls132015}. We will use the term “TLS” in the remainder of this survey.

%Based on this history, we will refer as TLS in the rest of survey.

\subsection{Overview of TLS}
TLS operates below the Application layer and above Transport layer, as illustrated in Figure \ref{tlssublayer}. 
%In this work, by the term \textit{Application} we mean the top-level applications such as Web, Mail, VoIP and use the term \textit{Protocol} to indicate how packets are exchanged between client and server. 
TLS contains two layers, the top-layer holds three protocols: (1) the Handshake protocol is responsible for negotiation to establish or resume a secure connection; (2) the Change Cipher Specification manages the modifications in the ciphering parameters, such as the ciphering algorithm; (3) the SSL Alert Protocol signals problems with SSL connections and allows the communicating peers to exchange alert messages. The lower-layer holds the Record protocol, which can be presented as an envelope for application data and TLS messages from the protocols above. The Record protocol is responsible for splitting data into fragments, which are optionally compressed, authenticated with a Message Authentication Code (MAC), encrypted and finally transmitted \cite{oppliger2009ssl}. 

%\begin{figure}[hbtp]
%\setlength{\belowcaptionskip}{-5pt}
%\centering
%\includegraphics[scale=0.5]{images/TLS-OSI-bw.eps}
%\caption{The TLS Layers and sub-protocols}
%\label{tlssublayer}
%\end{figure}

%In this work, we give more details about the TLS Handshake protocol since it has been used in the context of HTTPS monitoring as we will discuss. 
The Handshake protocol is of prime importance because it defines the first interactions and is responsible for many configuration aspects such as managing cipher suite negotiation, server/client authentication, and session key exchange. During cipher suite negotiation, client and server %make agreement about the cipher suite that will be used to exchange data. 
agree on a cipher suite that will be used to exchange data. 
In authentication, both parties prove their identity using Public Key Infrastructure (PKI) method. In the session key exchange, client and server exchange random and special numbers, called the Pre-Master Secret. These numbers are used to create their Master Secret, which will be used as key for encryption in the phase of exchanging data \cite{tls2016, oppliger2009ssl}. Figure \ref{tlshandshake} details the sequence of TLS Handshake protocol messages:
\begin{enumerate}
\item \texttt{ClientHello} message contains the usable cipher suites, supported extensions and a random number.
\item \texttt{ServerHello} message holds the selected cipher, supported extensions and a random number.
\item \texttt{ServerCertificate} message contains a certificate with the server public key.
\item \texttt{ServerHelloDone} indicates the end of the Server-Hello and associated messages. If the client receives a request for its certificate, it sends a \texttt{ClientCertificate} message. 
\item Based on the server random number, the client generates a random Pre-Master Secret, encrypts it with the public key given in the server's certificate and sends it to the server.
\item Both client and server generate a master secret from the Pre-master secret and exchanged random values. 
\item The client and server exchange \texttt{ChangeCipherSpec} to start using the new keys for encryption.
\item The client sends \texttt{Finished} message to verify that the key exchange and authentication processes were successful.
\item Server sends \texttt{Finished} message to the client.
\end{enumerate}

Once both sides have received and validated the \texttt{Finished} message from its peer, they can send and receive application data over the new TLS connection.

\subsection{Introduction to HTTPS protocol}
HTTPS is a protocol providing secure web communications. It simply consists in the Hypertext Transfer Protocol (HTTP) running within a secured TLS connection. To differentiate both services, HTTP uses the port 80 by default while HTTPS uses the port 443. Encrypted-HTTP traffic is still possible without HTTPS but is fundamentally different. A user who needs privacy can still access the desired website over VPN, SSH tunnel, ToR or SSL Proxy. In such case, the website's URL starts with "http://", which means that the web server does not provide a secure connection by itself and that the secure link parameters are configured within the chosen method, but not in the remote server. In HTTPS, the website's URL starts with "https://" and the website is hosted on an authenticated server that owns a SSL certificate. Thus, client and server negotiate the secure connection parameters before exchanging data thanks to HTTP over a dedicated secure link between them \cite{miller2014know}.

==> discussion.tex <==
In this paper, we have tackled the real-time identification of HTTPS services. We have proposed a novel approach to identify services based on the TLS handshake packets and a few number of application data packets. The results show that we can identify HTTPS services using the TLS handshake packet and up to 9 application data packets without loosing accuracy. So we need at most 13 packets (4 TLS handshake packets + 9 application data packets) to recognize the HTTPS service behind a flow, what is very early in the session compared to others values in related work that need 70 or 100 packets. 

The findings of this work can be considered from different sides. From one side, we can identify HTTPS services in real-time by using a small number of application data packets in addition to the TLS handshake packets. From another side, we can also consider to have a trade-off between security and accuracy by tuning the threshold value. So if accessing to a forbidden service generates a high risk, then we can set the model to identify services using only handshake packets to prevent any exchange of application data packets, even if this configuration may affect other legitimate services due to its lower accuracy. On the opposite, for other kinds of application focused on QoS or accounting, for example while monitoring video streaming or file download over HTTPS connections that generate long flows, we may consider more packets for identification, the small amount of data exchanged being considered less critical. Hence, by using 9 application data packets these services can be detected with approximately 92 \% accuracy. We achieved a similar accuracy as in \cite{schatzmann2010digging} (93\%) to identify services in HTTPS, but we do it in real-time, and we identify many types of services, not just web-mail ones. So we consider that this contribution significantly improve to the state-of-the-art of HTTPS monitoring approaches.

For the security point of view, if we use 9 application data packets to gain a higher accuracy, the amount of leaked data is still expected and under control. After removing the headers, the payload of a TCP data packet is 1460 Bytes. So up to 13 kB (9*1460) can be exchanged overall. But based on our dataset, we found that the average size of the encrypted payload transmitted from client to server is only 306 Bytes, and 331 Bytes in the opposite direction. Hence, if we allow 9 application data packets to be exchanged, the average amount of data will be in reality around (9*318) Bytes or 2.8 kB, before we are able to identify the flow and to decide if the flow is allowed or not. 

==> roc.tex <==
%\pgfplotstableread{Results/ROC/0.csv}
%\roczero
%\pgfplotstableread{Results/ROC/1.csv}
%\rocone
%\pgfplotstableread{Results/ROC/2.csv}
%\roctwo
%\pgfplotstableread{Results/ROC/3.csv}
%\rocthree
%\pgfplotstableread{Results/ROC/4.csv}
%\rocfour
%\pgfplotstableread{Results/ROC/9.csv}
%\rocnine
%  
%\begin{figure}[t]
%%\textbf{\setlength{\belowcaptionskip}{-10pt}}
%
%\centering
%\mbox {
%%\subfloat[ROC curve for classification model using one data packet]{\begin{tikzpicture}[.style={fill=none}]
%%\begin{axis}[
%%baseline,
%%trim axis left,
%%trim axis right,grid=major,
%%%legend style={at={(0.6,0.3)}, anchor=north,font=\tiny},
%%%xmin=0,xmax=0.05,  
%%%ymin=0.8,ymax=1,
%%xlabel= FPR,
%%ylabel= TPR, ylabel absolute, ylabel style={yshift=-0.6cm},
%%tick label style={font=\tiny},  xmin=-0.01,xmax=0.15,grid=major,
%%ymin=0.9,ymax=1,
%%label style={font=\tiny},
%%height=4.5cm,width=4.5cm]
%%\addplot[color=blue,mark=diamond]  table from \rocone;
%%%\addplot[color=violet,mark=square]  table from \rocnine;
%%\end{axis}
%%%\node[pin=30:{%
%%%    \begin{tikzpicture}[baseline,trim axis left,trim axis right]
%%%    \begin{axis}[
%%%        tiny,grid=major,
%%%      xmin=-0.01,xmax=0.01,
%%%      ymin=0.95,ymax=1,
%%%      enlargelimits,
%%%    ]
%%%    \addplot[color=blue,mark=diamond]  table from \rocone;
%%%\end{axis}
%%%    \end{tikzpicture}%
%%%}] {};
%%\label{rocone}
%%\end{tikzpicture}
%%}
%%\quad
%%\subfloat[ROC curve for classification model using nine data packets]{
%\begin{tikzpicture}[.style={fill=none}]
%\begin{axis}[
%baseline,
%%trim axis left,
%%trim axis right,grid=major,
%legend style={at={(0.65,0.25)}, anchor=north,font=\tiny},
%xlabel= FPR,
%ylabel= TPR, ylabel absolute, ylabel style={yshift=-0.6cm},
%tick label style={font=\tiny},
%label style={font=\tiny}, xmin=-0.01,xmax=0.2,grid=major,
%ymin=0.975,ymax=1,
%height=5.5cm,width=6cm]
%\addplot[color=red,mark=square]  table from \rocnine;
%\addplot[color=blue,mark=diamond]  table from \rocone;
%\legend{9 Application data packets, 1 Application data packet}
%\end{axis}
%%\label{rocnine}
%
%\end{tikzpicture}
%%}
%}
%\caption{ROC curve for C4.5 classification models with one and nine application data packets}
%\label{roc}
%\end{figure} 

